Regression Discontinuity Design with Many Thresholds

Numerous empirical studies employ regression discontinuity designs with multiple cutoffs and heterogeneous treatments. A common practice is to normalize all the cutoffs to zero and estimate one effect. This procedure identifies the average treatment effect (ATE) on the observed distribution of individuals local to existing cutoffs. However, researchers often want to make inferences on more meaningful ATEs, computed over general counterfactual distributions of individuals, rather than simply the observed distribution of individuals local to existing cutoffs. This paper proposes a consistent and asymptotically normal estimator for such ATEs when heterogeneity follows a non-parametric function of cutoff characteristics in the sharp case. The proposed estimator converges at the minimax optimal rate of root-n for a specific choice of tuning parameters. Identification in the fuzzy case, with multiple cutoffs, is impossible unless heterogeneity follows a finite-dimensional function of cutoff characteristics. Under parametric heterogeneity, this paper proposes an ATE estimator for the fuzzy case that optimally combines observations to maximize its precision.

==> assumptions.tex <==





%<*assu00A>
\begin{assumption}[Pooling]\label{assu_pool}
For any $\{ d,d' \} \subset \m{D}$, the conditional expectation 
\[
\mme\left[ \mmy(X_{i,p},d',U_{i,p}) - \mmy(X_{i,p},d,U_{i,p}) ~|~ X_{i,p}=x\right]
\]
as a function of $x$ does not depend on $p$.
\end{assumption}
%</assu00A>


%<*assu00AB>
\begin{assumption}[Policy Invariance]\label{assu_poli}
Regardless of the distribution of $(X_i,D_i,U_i)$ in a counterfactual policy, individual outcomes are always generated by a fixed response function $\mmy$, that is,
$Y_i = \mmy(X_{i},D_i,U_{i})$.
\end{assumption}
%</assu00AB>




%<*assu00B>
\begin{assumption}\label{assu_srd_est_kernel}
The kernel density function $k:\mathbb{R}\to\mathbb{R}$ is symmetric around zero, has compact support $[-M,M]$
for some $M \in (0,\infty)$,
and is Lipschitz continuous.
\end{assumption}
%</assu00B>


%<*assu00C>
\begin{assumption}\label{assu_srd_est_fx}
 \textbf{(a)}The distribution of $X_i$ has probability density function $f(x)$ that is continuous
 and has bounded support
 $\m{X}=[\underline{ \m{X}},\overline{ \m{X}}]$;
 \textbf{(b)}$f(x)$ is differentiable with bounded derivative $\nabla_x f(x)$.
\end{assumption}
%</assu00C>




%<*assu00D>
\begin{assumption}\label{assu_srd_est_mx}
Let $\rho_1 \in \mathbb{Z}_+$ be the order of the first-step LPR.
For arbitrary $d \in \m{D}$,
\textbf{(a)}$R(x,d)=\mme[Y_i(d)|X_i=x]$ is $\rho_1+1$
  times continuously differentiable wrt $~x$;
   its $(\rho_1+1)$-th partial derivative wrt $~x$ is denoted as $\nabla_x^{\rho_1+1} R(x,d)$;
\textbf{(b)}$\sigma^2(x,d)= \mmv \left[ Y_i(d) | X_i=x \right]$
 where $\mmv$ is the variance operator;
$\sigma^2(x,d)$ is continuously
 differentiable wrt $~x$; its  partial derivative wrt $~x$ is denoted as $\nabla_x \sigma^2(x,d)$;
 $\sigma^2(x,d)$ is bounded away from zero, and 
 $\mme[| Y_i(d) - R(X_i,d) |^3 | X_i ]$ is bounded.
\end{assumption}
%</assu00D>



%<*assu00E>
\begin{assumption}\label{assu_srd_kinf_est_cut}
\textbf{(a)}The schedule of cutoffs and doses comes
from a triangular array of fixed constants
$\m{C}_{K_n}= \left\{ \boup{c}_{j,n} \right\}_{ j =1 }^{K_n}$
that depends on the sample size $n$;
$\m{C}_{K_n}$ converges to a countably infinite set $\m{C}_{\infty}$ as $n \to \infty$;
$\m{C}_{\infty}$ is dense in its convex hull $\m{C}$;
\textbf{(b)}given the first-step bandwidth sequences $h_{1j,n}$, assume that
$c_{j,n}+h_{1j,n}<c_{j+1,n}$ and
$c_{j,n} \leq c_{j+1,n} - h_{1j+1,n}$
for all $j=1,\ldots, K_n-1$;
and
\textbf{(c)}given the second-step bandwidth sequence $h_{2,n}$ 
and polynomial order $\rho_2$,
define  $\boup{E}_n(\boup{c})$ 
  and $\bOmg_n(\boup{c};h_{2,n})$ as in
Equations \eqref{eq_est_int_Omg}-\eqref{eq_est_int_E} for each $n$.
Assume there exists a positive definite $J \times J$ matrix $\bQ$ such that%\\[-1cm]
\begin{gather*}
  \sup\limits_{ \boup{c} \in \m{C} }
  \left\|
  K_n h_{2,n}^3
  \left[ \boup{E}_n(\boup{c}/h_{2,n})' \bOmg_n(\boup{c};h_{2,n}) \boup{E}_n(\boup{c}/h_{2,n}) \right]^{-1}
  - \bQ
  \right\|
   =o \left( 1 \right).
  % \\[-1cm]
\end{gather*}
\end{assumption}
%</assu00E>




%<*assu00F>
\begin{assumption}\label{assu_srd_kinf_est_int}
\textbf{(a)}$R(x,d) = \mme[Y_i(d)|X_i=x]$ 
 is a $\bar{\rho}$ times continuously differentiable function with
 $\bar{\rho} = \max\{\rho_1+2, \rho_2+2 \} $,
 where $\rho_1$ and $\rho_2$ are polynomial degrees in the first and second steps;
 the $\bar{\rho}$-th partial derivative of $R(x,d)$ with respect to $x$
  is denoted
 $\nabla_x^{\bar{\rho}} R(x,d)$;
\textbf{(b)} $\sigma^2(x,d) = \mmv[Y_i(d)|X_i=x]$ 
 is a continuous function bounded away from zero;
 and
\textbf{(c)} $\exists M \in (0,\infty)$ such that $\mmp[|Y_i(d) - R(X_i,d)| < M]=1$ for $\forall d \in \m{D}$.
\end{assumption}
%</assu00F>




%<*assu00G>
\begin{assumption}\label{assu_srd_id_param}
Let $\boup{\m{W}}(c,d)=[\m{W}_1(c,d), \allowbreak \ldots, \m{W}_q(c,d)]'$
be a vector-valued function $\boup{\m{W}}:\m{X} \times \m{D} \to \mathbb{R}^{q \times 1}$
known to the researcher and such that
\textbf{(a)} $\mme_{F} \left[\boup{\m{W}}(c,d')-\boup{\m{W}}(c,d) \right]$
is well-defined for the counterfactual distribution $F$;
and
\textbf{(b)} $\m{W}_j(c,d') - \m{W}_j(c,d)$, $j=1,\ldots,q$, are linearly independent functions.
The treatment effect function $\beta_{ec}(\bc)$ is assumed to belong to the following class
of functions:
\begin{gather*}
\m{H}
=\bigg\{
\beta: \m{C} \to \mmr ~:~ \beta(c,d,d') = \left[\boup{\m{W}}(c,d')-\boup{\m{W}}(c,d) \right]'
\boup{\theta} \text{, for }  \boup{\theta} \in \mmr^q
\bigg\}.
%\\[-1.25cm]
\end{gather*}
\end{assumption}
%</assu00G>



%<*assu00H>
\begin{assumption}\label{assu_frd_id_nodef}
\textbf{(a)}There are no ever-defiers: $\mmp[\mathbf{G}_{ed}]=0$;
\textbf{(b)}for arbitrary $d \in \m{D}$, and $\bar{\m{U}} \in \m{U}^*$,
%defined in Eq. \ref{eq_def_ustar},
$\mme[ Y_i(d) | X_i=x, {\m{U}_i} = \bar{\m{U}} ]$ and $\mmp\left[{\m{U}_i} = \bar{\m{U}} | X_i=x \right]$
    are continuous and bounded functions of $x$;
\textbf{(c)} there exists a function $\beta_{ec}(\boup{c})$ such that  
    $  \mme[Y_i(d')-Y_i(d)|X_i=c, {\m{U}_i} = \bar{\m{U}} ] =  \beta_{ec}(\boup{c}) $ for every $\bc=(c,d,d') \in \m{C}$ and  $\bar{\m{U}} \in \mathbf{G}_{ec}$.
    \end{assumption}
%</assu00H>



%<*assu00I>
\begin{assumption}\label{assu_frd_est_mx}
For any $d \in \m{D}$, and
any $\bar{\m{U}}$ in the class $\m{U}^*$ defined in Eq. \eqref{eq_def_ustar},
\textbf{(a)}$\mme[Y_i(d) |X_i=x, \m{U}_i =  \bar{\m{U}} ]$ is a ${\rho_1}+1$  times continuously differentiable function of $~x$
 with $({\rho_1}+1)$-th derivative $\nabla_x^{{\rho_1}+1} \mme[Y_i(d) |X_i=x, \m{U}_i =  \bar{\m{U}}]$;
\textbf{(b)}$\mmv[Y_i(d)^{2}|X_i=x,  \m{U}_i =  \bar{\m{U}} ]$ is a continuous function of $x$,
and 
$\mme \left[ \left| Y_i(d) -  \mme[Y_i(d) |X_i=x, \m{U}_i =  \bar{\m{U}} ] \right|^3 ~|~X_i=x,  \m{U}_i =  \bar{\m{U}} \right]$
is bounded;
\textbf{(c)}for $\widetilde{\boup{W}}$ defined in Eq. \eqref{eq_def_Wtilde},
  $\widetilde{\boup{W}}' \widetilde{\boup{W}}$ is invertible;
\textbf{(d)}$\mmp[ \m{U}_i =  \bar{\m{U}} | X_i=x]$ is a $\rho_1+1$ times continuously differentiable function of $~x$
 with $(\rho_1+1)$-th derivative $\nabla_x^{\rho_1+1} \mmp[ \m{U}_i =  \bar{\m{U}} | X_i=x]$.
\end{assumption}
%</assu00I>





%\end{document} 
